Animal Identification with Independent Foreground and Background Modeling

We propose a method that robustly exploits background and foreground in visual identification of individual animals. Experiments show that their automatic separation, made easy with methods like Segment Anything, together with independent foreground and background-related modeling, improves results. The two predictions are combined in a principled way, thanks to novel Per-Instance Temperature Scaling that helps the classifier to deal with appearance ambiguities in training and to produce calibrated outputs in the inference phase. For identity prediction from the background, we propose novel spatial and temporal models. On two problems, the relative error w.r.t. the baseline was reduced by 22.3% and 8.8%, respectively. For cases where objects appear in new locations, an example of background drift, accuracy doubles.

==> sections/4_datasets.tex <==
\section{Datasets}
\label{sec:datasets}



\subsection{Eurasian lynx}
\label{sec:lynx}

 

\subsection{Loggerhead sea turtle}
\label{sec:turtles}



% \begin{figure}[!b]
%  \centering
% \begin{tikzpicture}[font=\small]
% \begin{axis}[
%       width=\linewidth,
%       xmin=0,
%       xmax=438,
%       ymin=0,
%       ymax=190,
%       title={},
%       xlabel={\# of unique individuals},
%       ylabel={\# of photographs},
%       ylabel near ticks,
%       height=130,
% ]
%       \addplot [mark=none, very thick, myblue] table[x index=0, y index=1] {\dataTurtleCounts}; 
% \end{axis}
% \end{tikzpicture}
% \caption{Number of photographs for each of the 438 turtles.}
%  \label{fig:individuals2}
% \end{figure}

% \begin{figure}[!b]
%  \centering
% \begin{tikzpicture}[font=\small]
% \begin{axis}[
%       width=\linewidth,
%       xmin=0,
%       xmax=105,
%       ymin=0,
%       ymax=625,
%       title={},
%       xlabel={\# of unique individuals},
%       ylabel={\# of photographs},
%       ylabel near ticks,
%       height=130,
% ]
%       \addplot [mark=none, very thick, mygreen] table[x index=0, y index=1] {\dataLynxCounts}; 
%       \addplot [dashed, very thick, myorange] (1,10) -- (450,10);
% \end{axis}
% \end{tikzpicture}
% \caption{Number of photographs for each of the 102 lynxes (green). }
%  \label{fig:individuals3}
% \end{figure}


% \begin{figure}[!t]
% \begin{minipage}{\linewidth}
% \centering
%     \includegraphics[height=21cm]{figures/dist/dist-lynxes.pdf} \\
% \caption{Number of photographs for each of the 102 lynxes. }
%  \label{fig:individuals4}
% \end{minipage}
% \end{figure}

==> tables/lynx-old.tex <==
\begin{table*}     
\centering
\begin{tabular}{l|ccc}
\toprule
 & No explicit prior & Fixed location prior & Moving location prior\\
\midrule
Crop & 49.05 & 55.45 \\
Foreground mask & 50.47 & 57.79 \\
Foreground mask + per-instance calibration & 53.07 & 59.22 & 60.53\\
Foreground mask + erosion 3px & 48.66 & 56.46  \\
Foreground mask + erosion 5px & 47.87 & 55.26 \\
Background mask & 24.90 & \\
\bottomrule
\end{tabular}
\caption{Lynx identification accuracy}
\label{tab:lynx}
\end{table*}

==> tables/segmentationablation.tex <==
\begin{table}
  \small
  \setlength{\tabcolsep}{0.85em}
  % \setlength\tabcolsep{2pt}
  \centering
  \caption{Segmentation method ablation on the Eurasian lynx dataset.}
  \vspace{-7pt}
  \begin{tabular}{@{}lcc|cc@{}}
    \toprule          
    Input & Loss & Background model $\Psi_k$ &  SAM~\cite{kirillov2023segany} & Human \\
    \midrule    
    Foreground & CE &-- &49.3\% & 48.3\% \\ 
    Background & CE & -- & 27.1\% & 25.6\%  \\ 
    Foreground & PITS & -- & 52.5\% & 50.6\% \\     
    Foreground + $\Psi_k$ & PITS & $\text{HL}_\theta$ & 59.7\% & 56.6\% \\
    Foreground + $\Psi_k$ & PITS & $\text{ML}_\theta$ & 60.9\% & 57.1\% \\ 
    \bottomrule
  \end{tabular}
  
  \label{tab:segmentationablation}
\end{table}

